DublinCity: Annotated LiDAR Point Cloud and its Applications

Scene understanding of full-scale 3D models of an urban area remains a challenging task. While advanced computer vision techniques offer cost-effective approaches to analyse 3D urban elements, a precise and densely labelled dataset is quintessential. The paper presents the first-ever labelled dataset for a highly dense Aerial Laser Scanning (ALS) point cloud at city-scale. This work introduces a novel benchmark dataset that includes a manually annotated point cloud for over 260 million laser scanning points into 100'000 (approx.) assets from Dublin LiDAR point cloud [12] in 2015. Objects are labelled into 13 classes using hierarchical levels of detail from large (i.e., building, vegetation and ground) to refined (i.e., window, door and tree) elements. To validate the performance of our dataset, two different applications are showcased. Firstly, the labelled point cloud is employed for training Convolutional Neural Networks (CNNs) to classify urban elements. The dataset is tested on the well-known state-of-the-art CNNs (i.e., PointNet, PointNet++ and So-Net). Secondly, the complete ALS dataset is applied as detailed ground truth for city-scale image-based 3D reconstruction.

==> suppl_mat_3Dreconst-SR.tex <==
\subsection*{Image-based 3D reconstruction evaluation}
%\subsubsection*{Aerial imagery description}
%The LiDAR point cloud acquisition was the primary output of the aerial scanning. However, the helicopter also collected imagery during the flight~\cite{laefer20172015}. In this supplementary material, the two sets of images used in the paper are detailed.

%\textbf{Top view imagery}.\label{subsec:GeoRegisteredRGB} The dataset includes 4471 images taken from a helicopter an are called in the cited repository as Geo-referenced RGB. The resolution in pixels of the images is $9000\times6732$ and are stored in TIFF format, with a ground sampling distance of 3.4 cm. The total size of the images is 813 GB and they are presented in the different flight paths. The geographic information is given as GPS tag in the EXIF metadata and the camera used for the capture is Leica RCD30. 

%\textbf{Oblique view imagery}.\label{subsec:ObliqueImagery} The oblique imagery contains 4033 JPEG images which are taken with two different NIKON D800E cameras. They are referred to as Oblique photos, their resolution is $7360\times4912$ and its size is 18.5 GB. As it happens with geo-registered RGB images, they are presented in accordance with the flight path but including an extra subdivision which corresponds to each camera.

\subsubsection*{Additional figures}
\begin{figure}[!h]
    \centering
    %[width=0.35\linewidth] [width=0.50\linewidth]
    \includegraphics[width=0.48\linewidth]{figures/3dRecons/suppl_mat/oblique_tiles.png}
    \includegraphics[width=0.48\linewidth]{figures/3dRecons/suppl_mat/rgb_tiles.png}
    \caption{Image-based reconstruction in the overlapping area. On the left, the result with the oblique view imagery; on the right, with the top view imagery}
    \label{fig:3dRecons:suppl_mat}
\end{figure}
\begin{figure}[!h]
    \centering
    %[width=0.35\linewidth] [width=0.50\linewidth]
    \includegraphics[width=0.24\linewidth]{figures/3dRecons/suppl_mat/ICP_registration/before_ICP_oblique_detail.png}
    \includegraphics[width=0.24\linewidth]{figures/3dRecons/suppl_mat/ICP_registration/before_ICP_oblique_2_detail.png}
    \includegraphics[width=0.24\linewidth]{figures/3dRecons/suppl_mat/ICP_registration/before_ICP_RGB_detail.png}
    \includegraphics[width=0.24\linewidth]{figures/3dRecons/suppl_mat/ICP_registration/before_ICP_RGB_2_detail.png}
    \\
    \includegraphics[width=0.24\linewidth]{figures/3dRecons/suppl_mat/ICP_registration/after_ICP_oblique_detail.png}
    \includegraphics[width=0.24\linewidth]{figures/3dRecons/suppl_mat/ICP_registration/after_ICP_oblique_2_detail.png}
    \includegraphics[width=0.24\linewidth]{figures/3dRecons/suppl_mat/ICP_registration/after_ICP_RGB_detail.png}
    \includegraphics[width=0.24\linewidth]{figures/3dRecons/suppl_mat/ICP_registration/after_ICP_RGB_2_detail.png}
    \caption{Top row shows some details of the reconstruction with the coarse registration done with the GPS data. Second row, shows the same details after ICP registration. LiDAR point cloud, reconstruction with oblique images and reconstruction with top view images are shown in yellow, cyan and blue, respectively. }
    \label{fig:3dRecons:suppl_mat:ICP_registration}
\end{figure}
%\begin{figure}
%    \centering
%    \includegraphics[width=0.32\linewidth]{figures/3dRecons/FscoreRecallPrecision/F_score_RGB.pdf}
%     \includegraphics[width=0.32\linewidth]{figures/3dRecons/FscoreRecallPrecision/Recall_RGB.pdf}
%     \includegraphics[width=0.32\linewidth]{figures/3dRecons/FscoreRecallPrecision/Precision_RGB.pdf}
%     
%    \includegraphics[width=0.32\linewidth]{figures/3dRecons/FscoreRecallPrecision/F_score_oblique.pdf}
%     \includegraphics[width=0.32\linewidth]{figures/3dRecons/FscoreRecallPrecision/Recall_oblique.pdf}
%     \includegraphics[width=0.32\linewidth]{figures/3dRecons/FscoreRecallPrecision/Precision_oblique.pdf}
%    \caption{F-score, recall and precision of the image-based reconstruction (from left to right) per tile. The top row shows the results of the top view images reconstruction and the bottom one, the results with the oblique view ones. The values given per tile corresponds with the value of the curves at a given precision (dash line)}
%    \label{fig:3dRecons:FscoreRecallPrecision}
%\end{figure}
%% just in case it is needed
%\begin{figure}
%    \centering
%    \includegraphics[width=0.75\linewidth]{figures/3dRecons/suppl_mat/reconstruction_to_be_segmented.png}
%    \includegraphics[width=0.48\linewidth]{figures/3dRecons/suppl_mat/lidar.png}
%    \includegraphics[width=0.48\linewidth]{figures/3dRecons/suppl_mat/3d_Recons_facades.png}
%    \caption{On the top, a section of 250 $m^2$ of the image-based 3D reconstruction with RGB images. At the bottom, some facades are segmented from this area thanks to the annotation of our DublinCity database (in yellow).}
%    \label{fig:3dRecons:segmentation}
%\end{figure}
